How Does Language Influence Documentation Workflow? Unsupervised Word Discovery Using Translations in Multiple Languages

For language documentation initiatives, transcription is an expensive resource: one minute of audio is estimated to take one hour and a half on average of a linguist's work (Austin and Sallabank, 2013). Recently, collecting aligned translations in well-resourced languages became a popular solution for ensuring posterior interpretability of the recordings (Adda et al. 2016). In this paper we investigate language-related impact in automatic approaches for computational language documentation. We translate the bilingual Mboshi-French parallel corpus (Godard et al. 2017) into four other languages, and we perform bilingual-rooted unsupervised word discovery. Our results hint towards an impact of the well-resourced language in the quality of the output. However, by combining the information learned by different bilingual models, we are only able to marginally increase the quality of the segmentation.

==> results_table.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{lcc|ccccc|c}
\hline
           &             & \textbf{Bilingual} & \multicolumn{5}{c|}{\textbf{Multilingual Voting}}                                & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{ANE Selection}}} \\ \cline{1-3}
\textbf{1} & \textbf{FR} & \textbf{73.40}     &                    & \textbf{0.25} & \textbf{0.5}   & \textbf{0.75} & \textbf{1} & \multicolumn{1}{l}{}                                        \\ \cline{4-9} 
\textbf{2} & \textbf{EN} & 73.10              & \textbf{(1-2)}     & 73.10         & 73.10          & 73.30         & 73.30      & 73.80                                                       \\
\textbf{3} & \textbf{ES} & 72.60              & \textbf{(1-3)}     & 72.40         & 74.60          & 72.10         & 72.10      & \textbf{73.90}                                              \\
\textbf{4} & \textbf{PT} & 72.80              & \textbf{(1-4)}     & 71.60         & 74.80          & 74.20         & 70.90      & 73.90                                                       \\
\textbf{5} & \textbf{DE} & 71.00              & \textbf{ALL (1-5)} & 74.30         & \textbf{74.90} & 73.10         & 70.00      & 73.90                                                      
\end{tabular}
\end{table}

==> top_types.tex <==

\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll|ll|ll|ll|ll}
\hline
\multicolumn{2}{c|}{\textbf{MB-DE}} & \multicolumn{2}{c|}{\textbf{MB-EN}} & \multicolumn{2}{c|}{\textbf{MB-ES}} & \multicolumn{2}{c|}{\textbf{MB-FR}} & \multicolumn{2}{c}{\textbf{MB-PT}} \\\hline
itua            & itoua            & ibara            & ibara           & ingobha           & ingobha        & itua             & itoua           & oboá+ngá         & oboa            \\
mωndzω          & monzo            & otsέngε          & otsenge         & ondóngo           & ondongo        & itúa+ngá         & itoua           & ERROR            & nyaamvua        \\
tsimba          & tsimba           & asúa             & asoua           & mbía+mbvúlá       & amvoulou       & itúa+mbía        & itoua           & itua             & itoua           \\
abia            & Freunde          & okúmú            & okoumou         & itua              & itoua          & kánga            & pintade         & mbembe           & mbembe          \\
tsósá           & Henne            & olangi           & bottle          & y'+konga          & cuerno         & ERROR            & nyobhosi        & tsimba           & tsimba   \\\hline      
\end{tabular}
}
\caption{CAPTION HERE}
\label{tab:types}
\end{table}
